Inverse Mixed Integer Optimization: Polyhedral Insights and Trust Region Methods

Inverse optimization, determining parameters of an optimization problem that render a given solution optimal, has received increasing attention in recent years. While significant inverse optimization literature exists for convex optimization problems, there have been few advances for discrete problems, despite the ubiquity of applications that fundamentally rely on discrete decision-making. In this paper, we present a new set of theoretical insights and algorithms for the general class of inverse mixed integer linear optimization problems. Specifically, a general characterization of optimality conditions is established and leveraged to design new cutting plane solution algorithms. Through an extensive set of computational experiments, we show that our methods provide substantial improvements over existing methods in solving the largest and most difficult instances to date.

==> EC_Extra_ApproxQuality.tex <==

\section{Approximation quality of inverse linear optimization}


If $\mX$ is continuous and is represented as $\mX = \{\bx \ | \ \bA\bx \geq \bb\}$, then the inverse optimization problem can be solved as the following linear program \citep[e.g.][]{chan2018inverse}: 
\begin{subequations}
\begin{align*}
\textbf{IO}(\bc^0, \ix, \mX): \ \underset{\by,\bc}{\text{minimize}} \quad & ||\bc^0 - \bc||_1 \\
\text{subject to} \quad & \bA^\top \by = \bc,\\
& \bc^\top \ix = \bb^\top \by,\\
& \by \geq \mathbf{0}.
\end{align*}
\end{subequations}


The example bellow illustrates that solving a inverse linear optimization problem by relaxing integrality constraints cannot be used to approximate inverse MILO models.


\begin{ex}\label{ex:LP_approximation}
Consider model \ref{model:IOM-Bilevel1} with $\bc^0 = (-1,-1)$, $\ix = (0,1)$ and $\mX = \{b_1, b_2 \in \{0,1\} \ | \ b_1 + \frac{3}{5} b_2 \leq 1\}$. Let $\mX_{LP} = \{b_1, b_2 \in [0,1] \ | \ b_1 + \frac{3}{5} b_2 \leq 1\}$ represent the feasible region without the integrality constraints.


\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.48\textwidth}
\centering
  \begin{tikzpicture}%[>=latex]
    \begin{scope}
    \clip (-1,-0.5) rectangle (3cm,3cm); 
    \begin{scope}[transparency group]
    \begin{scope}[blend mode=multiply]
    \filldraw[fill=black!50, draw=black,opacity=0.1] (0,0) -- (2,0) -- (0,2) -- cycle; % Puts the shaded rectangle
    \end{scope}
    \end{scope}

    \draw[style=help lines, line width = 0.01mm,lightgray!60] (0,0) grid[step=2cm] (2,2); % Draws a grid in the new coordinates.



    \foreach \x in {0,2}{                           % Two indices running over each
        \foreach \y in {0,2}{                       % node on the grid we have drawn 
        \node[draw,circle,inner sep=0.01pt,fill,lightgray!60] at (\x,\y) {}; % Places a dot at those points
        }
    }
    %\node[above left] (x2) at (1,4) {\color{gray}$\bhx_2$};
    %\node[above left] (x3) at (2,5) {\color{gray}$\bhx_3$};
    \node[above left] (x) at (0,2) {$\ix$};
    \node[draw,circle,inner sep=0.8pt,fill,darkgray] at (0,2) {};
    
    \node[below left] (x) at (0,0) {$(0,0)$};
    \node[draw,circle,inner sep=0.8pt,fill,darkgray] at (0,0) {};
    
    \node[below right] (x) at (2,0) {$(1,0)$};
    \node[draw,circle,inner sep=0.8pt,fill,darkgray] at (2,0) {};
    

    \draw [-, line width = 0.05mm,darkgray] (0,4) -- (2.4,0);
    %--------lines --------
    %\node[draw,circle,inner sep=1pt,fill] at (1,5) {};
    %\node[above left] (x1) at (1,5) {$\bx_1$};


    \end{scope}
\end{tikzpicture}
\caption{$\conv(\mX)$}\label{fig:EC_example_strict}
\end{subfigure}
\hspace{-0.5cm}
\begin{subfigure}[t]{0.48\textwidth}
\centering
  \begin{tikzpicture}%[>=latex]
    \begin{scope}
    \clip (-1,-0.5) rectangle (3cm,3cm); 
    \begin{scope}[transparency group]
    \begin{scope}[blend mode=multiply]
    \filldraw[fill=black!50, draw=black,opacity=0.1] (0,0) -- (2,0) -- (2,0.7) -- (1.2,2)  -- (0,2) -- cycle; % Puts the shaded rectangle
    \end{scope}
    \end{scope}

    \draw[style=help lines, line width = 0.01mm,lightgray!60] (0,0) grid[step=2cm] (2,2); % Draws a grid in the new coordinates.


    \foreach \x in {0,2}{                           % Two indices running over each
        \foreach \y in {0,2}{                       % node on the grid we have drawn 
        \node[draw,circle,inner sep=0.01pt,fill,lightgray!60] at (\x,\y) {}; % Places a dot at those points
        }
    }
    \node[above left] (x) at (0,2) {$\ix$};
    \node[draw,circle,inner sep=0.8pt,fill,darkgray] at (0,2) {};
    
        \node[below left] (x) at (0,0) {$(0,0)$};
    \node[draw,circle,inner sep=0.8pt,fill,darkgray] at (0,0) {};
    
    \node[below right] (x) at (2,0) {$(1,0)$};
    \node[draw,circle,inner sep=0.8pt,fill,darkgray] at (2,0) {};
    
    %--------lines --------
    \draw [-, line width = 0.05mm,darkgray] (0,4) -- (2.4,0);
    %\node[draw,circle,inner sep=1pt,fill] at (1,5) {};
    %\node[above left] (x1) at (1,5) {$\bx_1$};


    \end{scope}
\end{tikzpicture}
\caption{$\conv(\mX_{LP})$}\label{fig:EC_example_relaxed}
\end{subfigure}
\end{figure}

Using figure \ref{fig:EC_example_strict}, it is easy to see that $\bc^0$ is the optimal solution to the inverse optimization problem, since $(\bc^0)^\top \bhx < 0$ (feasible point (0,0)) and $(\bc^0)\top < -1$ (feasible point (1,0)). On the other hand, solving the inverse optimization model with an LP approximation would give an optimal solution of $\bc^* = (0,-1)$ and an optimal value of $1$ unit. We can scale the values of $\bc^0$ to make this error arbitrarily large.


\end{ex}

==> EC_Extra_CPExample.tex <==

\begin{ex}\label{example:standardCP}
In this example, we illustrate the per-iteration outputs of the cutting plane algorithm over a 2-dimension integer forward-feasible region.  The convex hull of the forward-feasible region ($\conv(\mX)$) is shaded in gray.  Let $\ix = [4,5]$, $\ic = [5,-1]$, and recall that the objective of the master problem is $||\ic-\bc||_1$, i.e., $\sum_i |\ic_i - \bc_i|$. The set of discovered points is initialized as $\mhX^0 = \{\ix\}$.


\begin{figure}[!ht]
  \centering
      \scalebox{1}{
\begin{subfigure}[t]{0.31\textwidth}
\centering
  \begin{tikzpicture}[scale = 0.8]%[>=latex]
    \begin{scope}
    \clip (-0.7,0.7) rectangle (4.2cm,7.2cm); 
    \begin{scope}[transparency group]
    \begin{scope}[blend mode=multiply]
    \filldraw[fill=lightgray!30, draw=black,opacity=0.5] (0,0) -- (0,1) -- (1,4) -- (2,5) -- (4,6) -- (6,6) -- (6,0) -- cycle; % Puts the shaded rectangle
    \end{scope}
    \end{scope}

    \draw[style=help lines, line width = 0.01mm, lightgray] (-0,-0) grid[step=1cm] (7,7); % Draws a grid in the new coordinates.
    \draw[dashed, line width = 0.3mm, red] (-0,1) -- (4,6);

    \foreach \x in {0,1,...,7}{                           % Two indices running over each
        \foreach \y in {0,1,...,7}{                       % node on the grid we have drawn 
        \node[draw,circle,inner sep=0.5pt,fill, lightgray] at (\x,\y) {}; % Places a dot at those points
        }
    }
    \node[above left] (x1) at (0,1) {$\bhx^0$};
    %\node[above left] (x2) at (1,4) {\color{gray}$\bhx_2$};
    %\node[above left] (x3) at (2,5) {\color{gray}$\bhx_3$};
    \node[above left] (x) at (4,6) {$\ix$};
    \node[draw,circle,inner sep=1.2pt,fill] at (4,6) {};

    \draw [->, line width = 0.4mm] (4,1) -- (3,1.2);
    \draw [->, line width = 0.4mm, red, dashed] (4, 1) -- (3,1.8);

    \node (c0) at (2.4,1.3) {$\boldsymbol{-}\ic$};
    \node (c1) at (2.5,2.1) {\color{red}$\boldsymbol{-}\bc^1$};

    \end{scope}
\end{tikzpicture}
\caption{\vspace{0.5cm}$\mhX^1 = \{\bx^*, \bhx^0\}$}\label{subfig:it1}
\end{subfigure}
\begin{subfigure}[t]{0.31\textwidth}
\centering
  \begin{tikzpicture}[scale = 0.8]%[>=latex]
    \begin{scope}
    \clip (-0.7,0.7) rectangle (4.2cm,7.2cm); 
    \begin{scope}[transparency group]
    \begin{scope}[blend mode=multiply]
    \filldraw[fill=lightgray!30, draw=black,opacity=0.5] (0,0) -- (0,1) -- (1,4) -- (2,5) -- (4,6) -- (6,6) -- (6,0) -- cycle; % Puts the shaded rectangle
    \end{scope}
    \end{scope}

    \draw[style=help lines,line width = 0.01mm,lightgray] (-0,-0) grid[step=1cm] (14,14); % Draws a grid in the new coordinates.
    \draw[dashed, line width = 0.3mm, red] (1,4) -- (4,6);

    \foreach \x in {0,1,...,7}{                           % Two indices running over each
        \foreach \y in {0,1,...,7}{                       % node on the grid we have drawn 
        \node[draw,circle,inner sep=0.5pt,fill,lightgray] at (\x,\y) {}; % Places a dot at those points
        }
    }
    \node[above left] (x1) at (0,1) {$\bhx_0$};
    \node[above left] (x2) at (1,4) {$\bhx_1$};
    %\node[above left] (x3) at (2,5) {\color{gray}$\bhx_3$};
    \node[above left] (x) at (4,6) {$\ix$};
    \node[draw,circle,inner sep=1.2pt,fill] at (4,6) {};

    \draw [->, line width = 0.4mm] (4,1) -- (3,1.2);
    \draw [->, line width = 0.4mm, red, dashed] (4, 1) -- (3.4,1.9);

    \node (c0) at (2.4,1.3) {$\boldsymbol{-}\ic$};
    \node (c2) at (3,2.2) {\color{red}$\boldsymbol{-}\bc^2$};
    \end{scope}
\end{tikzpicture}
\caption{$\mhX^2 = \{\bx^*, \bhx^0, \bhx^1\}$}
\end{subfigure} \ \ 
\begin{subfigure}[t]{0.31\textwidth}
\centering
  \begin{tikzpicture}[scale = 0.8]%[>=latex]
    \begin{scope}
    \clip (-0.7,0.7) rectangle (4.2cm,7.2cm); 
    \begin{scope}[transparency group]
    \begin{scope}[blend mode=multiply]
    \filldraw[fill=lightgray!30, draw=black,opacity=0.5] (0,0) -- (0,1) -- (1,4) -- (2,5) -- (4,6) -- (6,6) -- (6,0) -- cycle; % Puts the shaded rectangle
    \end{scope}
    \end{scope}

    \draw[style=help lines,line width = 0.01mm,lightgray] (-0,-0) grid[step=1cm] (14,14); % Draws a grid in the new coordinates.
    \draw[dashed, line width = 0.3mm, red] (2,5) -- (4,6);

    \foreach \x in {0,1,...,7}{                           % Two indices running over each
        \foreach \y in {0,1,...,7}{                       % node on the grid we have drawn 
        \node[draw,circle,inner sep=0.5pt,fill, lightgray] at (\x,\y) {}; % Places a dot at those points
        }
    }
    \node[above left] (x1) at (0,1) {$\bhx^0$};
    \node[above left] (x2) at (1,4) {$\bhx^1$};
    \node[above left] (x3) at (2,5) {$\bhx^2$};
    \node[above left] (x) at (4,6) {$\ix$};
    \node[draw,circle,inner sep=1.2pt,fill] at (4,6) {};

    \draw [->, line width = 0.4mm] (4,1) -- (3,1.2);
    \draw [->, line width = 0.4mm, red, dashed] (4, 1) -- (3.5,2);

    \node (c0) at (2.4,1.3) {$\boldsymbol{-}\ic$};
    \node (c3) at (3.2,2.4) {\color{red}$\boldsymbol{-}\bc^{3}$};

    \end{scope}
\end{tikzpicture}
\caption{$\mhX^3 = \{\bx^*, \bhx^0, \bhx^1, \bhx^2\}$}
\end{subfigure}}
  \caption{The set of extreme points that are generated over the first three iterations of the pure cutting plane algorithm. Cuts from each newly discovered point is indicated using the red dashed link.}
\end{figure}


The cutting plane algorithm takes a total of four iterations, labeled by indices $0,1,2$ and $3$. The points $\bhx^0 = [0,0], \bhx^1 = [1,3], \bhx^2 = [2,4]$ and an unspecified $\bhx^3$ are generated with candidate vectors $\bc^0 = [5,-1]$, $\bc^1 = [5,-4]$, $\bc^2 = [2/3,-1]$, and $\bc^3 = [1/2,-1]$. The objective value of the inverse problem at each iteration is $3,4.33$, $4.5$ and $4.5$. The last point $\bhx_3$ (which is not shown) can be either $\bhx^2$ or $\ix$, both of which are optimal for $\bc^3$. Finally, in all iterations, only the last found point is binding at each iteration. Relate to certificate set
\end{ex}


We now apply the trust region enhanced cutting plane algorithm on the same problem. We use a simple trust-region updating function that does not modify the initial trust-region until no violated cuts are found, at which point the function returns $T^{k+1} := \mathbb{R}^N$ for all remaining iterations. 

\begin{ex}\label{example:CP-TR}

We apply the trust-region algorithm described above using three different initial trust-regions $\mT^0 = \{\bx \ s.t.\ ||\bx - \ix||_{\infty} \leq \delta\}$, where $\delta = 1,2,3$ in Figures \ref{subfig:example_TR1}, \ref{subfig:example_TR2}, and \ref{subfig:example_TR3}.

\begin{figure}[!ht]
  \centering
  \begin{subfigure}[t]{0.31\textwidth}
\centering
  \begin{tikzpicture}%[>=latex]
    \begin{scope}
    \clip (-0.7,0.7) rectangle (4.2cm,7.2cm); 
    \begin{scope}[transparency group]
    \begin{scope}[blend mode=multiply]
    \filldraw[fill=lightgray!30, draw=black,opacity=0.5] (0,0) -- (0,1) -- (1,4) -- (2,5) -- (4,6) -- (6,6) -- (6,0) -- cycle; % Puts the shaded rectangle
    \filldraw[fill = blue!8, line width = 0.4mm,opacity=0.5, draw = blue!50, dashed] (3,5) rectangle (5,7);
    \filldraw[fill=blue!14, draw=blue,opacity=0.6] (3,5) -- (3,5) -- (4,6) -- (6,6) -- (6,5) -- cycle;
    \end{scope}
    \end{scope}

    \draw[style=help lines,line width = 0.01mm,lightgray] (-0,-0) grid[step=1cm] (7,7); % Draws a grid in the new coordinates.
    %\draw[dashed, red] (-0,1) -- (4,6);

    \foreach \x in {0,1,...,7}{                           % Two indices running over each
        \foreach \y in {0,1,...,7}{                       % node on the grid we have drawn 
        \node[draw,circle,inner sep=0.5pt,fill,lightgray] at (\x,\y) {}; % Places a dot at those points
        }
    }
    \node[above left] (x1) at (2,5) {$\bhx_2$};
    \node[draw,circle,inner sep=1.2pt,fill] at (2,5) {};
    %\node[above left] (x2) at (1,4) {\color{gray}$\bhx_2$};
    %\node[above left] (x3) at (2,5) {\color{gray}$\bhx_3$};
    \node[above left] (x) at (4,6) {$\ix$};
    \node[draw,circle,inner sep=1.2pt,fill] at (4,6) {};
    \node[above left] at (3,5) {\color{blue}$\bhx_0$};
    \node[draw,circle,inner sep=1.2pt,fill,blue] at (3,5) {};

    %\draw [->, line width = 0.4mm] (3,5) -- (2.2,5.16);
    %\draw [->, line width = 0.4mm] (3,5) -- (2.5,5.5);
    \draw [->, line width = 0.4mm] (4,1) -- (3,1.2);
    \draw [->, line width = 0.4mm] (4,1) -- (3.1,1.9);
    \draw [->, line width = 0.4mm] (4,1) -- (3.5,2);
    %\draw [|->, line width = 0.4mm, red, dashed] (3.6, 1.4) -- (2.95,1.9);

    \node[above left] at (3.1,0.9) {$\boldsymbol{-}\bc^{\color{blue}0}$};
    \node[above left = 0.1cm and 0cm] at (3.3,1.7) {$\boldsymbol{-}\bc^{{\color{blue}1},2}$};
    \node[above left] at (4.2,2.0) {$\boldsymbol{-}\bc^{3}$};
    %\node (c1) at (2.7,2.2) {\color{red}$\bc^1$};

    \end{scope}
\end{tikzpicture}
\caption{TR of size 1}\label{subfig:example_TR1}
\end{subfigure}
\begin{subfigure}[t]{0.31\textwidth}
\centering
  \begin{tikzpicture}%[>=latex]
    \begin{scope}
    \clip (-0.7,0.7) rectangle (4.2cm,7.2cm); 
    \begin{scope}[transparency group]
    \begin{scope}[blend mode=multiply]
    \filldraw[fill=lightgray!30, draw=black,opacity=0.5] (0,0) -- (0,1) -- (1,4) -- (2,5) -- (4,6) -- (6,6) -- (6,0) -- cycle; % Puts the shaded rectangle
    \filldraw[fill = blue!8, line width = 0.4mm,opacity=0.5, draw = blue!50, dashed] (2,4) rectangle (6,8);
    \filldraw[fill=blue!14, draw=blue,opacity=0.6] (2,4) -- (2,5) -- (4,6) -- (6,6) -- (6,4) -- cycle;
    \end{scope}
    \end{scope}

    \draw[style=help lines,line width = 0.01mm,lightgray] (-0,-0) grid[step=1cm] (7,7); % Draws a grid in the new coordinates.
    %\draw[dashed, red] (-0,1) -- (4,6);

    \foreach \x in {0,1,...,7}{                           % Two indices running over each
        \foreach \y in {0,1,...,7}{                       % node on the grid we have drawn 
        \node[draw,circle,inner sep=0.5pt,fill,lightgray] at (\x,\y) {}; % Places a dot at those points
        }
    }
    %\draw [->, line width = 0.4mm] (3,5) -- (2.2,5.16);
    %\draw [->, line width = 0.4mm] (3,5) -- (2.5,5.5);
    \draw [->, line width = 0.4mm] (4,1) -- (3,1.2);
    \draw [->, line width = 0.4mm] (4,1) -- (3.5,2);
    %\draw [->, line width = 0.4mm] (3,2) -- (2.4,2.6);
    %\draw [->, line width = 0.4mm] (3,2) -- (2.6,2.8);
    %\draw [|->, line width = 0.4mm, red, dashed] (3.6, 1.4) -- (2.95,1.9);
    \node[above left] (x) at (4,6) {$\ix$};
    \node[draw,circle,inner sep=1.2pt,fill] at (4,6) {};
    \node[above left] at (2,5) {\color{blue}$\bhx_0$};
    \node[draw,circle,inner sep=1.2pt,fill,blue] at (2,5) {};
    
    \node[above left] at (3,0.9) {$\boldsymbol{-}\bc^{\color{blue}0}$};
    \node[above left] at (4.2,2) {$\boldsymbol{-}\bc^{{\color{blue}1},2}$};
    %\node[above left] at (3.2,2.8) {$\boldsymbol{-}\bc^3$};
    %\node (c1) at (2.7,2.2) {\color{red}$\bc^1$};

    \end{scope}
\end{tikzpicture}
\caption{TR of size 2}\label{subfig:example_TR2}
\end{subfigure}
\begin{subfigure}[t]{0.31\textwidth}
\centering
  \begin{tikzpicture}%[>=latex]
    \begin{scope}
    \clip (-0.7,0.7) rectangle (4.2cm,7.2cm); 
    \begin{scope}[transparency group]
    \begin{scope}[blend mode=multiply]
    \filldraw[fill=lightgray!30, draw=black,opacity=0.5] (0,0) -- (0,1) -- (1,4) -- (2,5) -- (4,6) -- (6,6) -- (6,0) -- cycle; % Puts the shaded rectangle
    \filldraw[fill = blue!8, line width = 0.4mm,opacity=0.5, draw = blue!50, dashed] (1,3) rectangle (6,8);
    \filldraw[fill=blue!14, draw=blue,opacity=0.6] (1,3) -- (1,4) -- (2,5)-- (4,6) -- (6,6) -- (6,3) -- cycle;
    \end{scope}
    \end{scope}

    \draw[style=help lines,line width = 0.01mm,lightgray] (-0,-0) grid[step=1cm] (7,7); % Draws a grid in the new coordinates.
    %\draw[dashed, red] (-0,1) -- (4,6);

    \foreach \x in {0,1,...,7}{                           % Two indices running over each
        \foreach \y in {0,1,...,7}{                       % node on the grid we have drawn 
        \node[draw,circle,inner sep=0.5pt,fill,lightgray] at (\x,\y) {}; % Places a dot at those points
        }
    }
    %\node[above left] (x1) at (0,1) {\color{gray}$\bhx_1$};
    %\node[above left] (x2) at (1,4) {\color{gray}$\bhx_2$};
    %\node[above left] (x3) at (2,5) {\color{gray}$\bhx_3$};
    \node[above left] (x) at (4,6) {$\ix$};
    \node[draw,circle,inner sep=1.2pt,fill] at (4,6) {};
    \node[above left] at (1,4) {\color{blue}$\bhx_0$};
    \node[draw,circle,inner sep=1.2pt,fill,blue] at (1,4) {};
    \node[above left] at (2,5) {\color{blue}$\bhx_1$};
    \node[draw,circle,inner sep=1.2pt,fill,blue] at (2,5) {};

    \draw [->, line width = 0.4mm] (4,1) -- (3,1.2);
    \draw [->, line width = 0.4mm] (4,1) -- (3,1.66);
    \draw [->, line width = 0.4mm] (4,1) -- (3.5,2);
    \node[above left] at (3,0.9) {$\boldsymbol{-}\bc^{\color{blue}0}$};
    \node[above left] at (3.1,1.5) {$\boldsymbol{-}\bc^{\color{blue}1}$};
    \node[above left] at (4.2,2) {$\boldsymbol{-}\bc^{{\color{blue}2},3}$};
    %\node[above left] at (3.2,2.8) {$\boldsymbol{-}\bc^3$};
    %\node (c1) at (2.7,2.2) {\color{red}$\bc^1$};

    \end{scope}
\end{tikzpicture}
\caption{TR of size 3}\label{subfig:example_TR3}
\end{subfigure}
\caption{\vspace{0.5cm} Illustration of the \CPTR \ algorithm using different trust-regions.}\label{fig:example_TR}
\end{figure}

In example \ref{subfig:example_TR1}, the points $\bhx^0 = [2,4], \bhx^2 = [3,4]$ and unspecified $\bhx^1$ and $\bhx^3$ are generated with candidate vectors $\bc^0 = [5,-1]$, $\bc^1 = \bc^2 = [3,-3]$ and $\bc^3 = [1/2,-1]$, giving objective values of $4,4, 4.5,  4.5$. In example \ref{subfig:example_TR2}, the points $\bhx^0 = [3,4]$ and an unspecified $\bhx^1$ and $\bhx^2$ are generated with candidate vectors $\bc^0 = [5,-1]$, $\bc^1 = \bc^2 = [1/2,-1]$, giving objective values of $4.5, 4.5, 4.5$. Finally, in example \ref{subfig:example_TR3}, the points $\bhx^0 = [1,3]$, $\bhx^1 = [2,4]$ and an unspecified $\bhx^2$ and $\bhx^3$ are generated with candidate vectors $\bc^0 = [5,-1]$, $\bc^1 = [2/3,-1]$ and $\bc^2 = \bc^3 = [1/2,-1]$ giving objective values of $4.33, 4.5, 4.5, 4.5$. We use the term unspecified $\bhx^k$ when both $\bhx^{k-1}$ and $\ix$ are possible solutions to the subproblem with candidate vector $\bc^k$.


\end{ex}



This example provides several important insights. First, we observe that the number of iterations required to solve the inverse problem in all three examples is at most equal to the number of iterations required for the pure cutting plane algorithm: example \ref{subfig:example_TR2} requires three iterations to solve the inverse problem, while examples \ref{subfig:example_TR1} and \ref{subfig:example_TR3} require four iterations each. 

In all three instances, the first iteration provides a better cut in the inverse space (since objective value with the cut is higher); in Figure \ref{subfig:example_TR1}, it is important to note that an \emph{interior point} of the set $\ext\{\conv\{\mX\}\}$ provided a better cut. This observation is important, since interior points can be otbtained with lower computational effort. Furthermore, the final objective value of $4.5$, first found at iteration $3$ in the pure cutting plane algorithm, is found at iterations $3$, $1$, and $2$ in examples \ref{subfig:example_TR1}, \ref{subfig:example_TR2}, \ref{subfig:example_TR3}, respectively. These two observations highlight that trust-regions may not only reduce per-iteration computational effort but may also reduce overall number of iterations.


==> EC_Extra_UnboundedInstances.tex <==

\section{Avoiding unbounded subproblems}\label{app:unbounded_subproblems}

It is possible for the master problem, which is a relaxation of the inverse problem, to propose a candidate cost vector which leads to an unbounded cut generation problem during iterations in which the trust region is removed. In particular, if $\mX$ is unbounded, then there exist $\bc$ vectors for which the cut generation problem $\textbf{FP}(\bc, \mX)$ is unbounded. Such candidate vectors are not inverse-feasible as mentioned by Remark \ref{rmk:Cbdd}, and thus need to be eliminated from the inverse problem relaxation. 

One way to accomplish this, as discussed in \citep{wang2009cutting}, is to the master problem with the following set of duality constraints,
\begin{equation}\label{eq:duality}
\by^\top \bA = \bc^\top, \ \by \geq \mathbf{0},
\end{equation}
noting that $\bA$ is the constraint coefficient matrix in the definition of the forward-feasible region $\mX$ (as seen in model \ref{model:FP}). With the duality constraints, the algorithm never proposes a candidate $\bc$ for which the forward problem $\min \{ \bc^\top \bx \ | \ \bx \in \mX \}$ becomes unbounded since for any $\bc$, the existence of $\by$ satisfying the duality constraints ensures that the dual of the LP relaxation of the forward problem, namely $\max \{ \bb^\top \by \ | \ \text{equations }  \eqref{eq:duality} \}$, is feasible, thus the primal LP, $\min \{ \bc^\top \bx \ | \ \bA \bx \geq \bb \}$ is bounded. The inverse model relaxation with duality constraints is then formulated as:
\begin{subequations}
\begin{align*}
\IOD(\mX): \ \ \underset{\bc,\mathbf{y}}{\text{minimize}} \quad & ||\ic-\bc|| \\
\text{subject to} \quad & \bc^\top (\ix - \bx) \leq 0, \quad \forall \ \bx \in \mX, \\
& \by^\top \bA = \bc^\top, \\
& \by \geq \mathbf{0}.
\end{align*}
\end{subequations}

\begin{rmk}
$\textup{\IOD}(\mX)$ is equivalent to $\textup{\IO}(\mX)$. 
\end{rmk}

 
Computationally, we find the additional of these constraints to the master problem to be burdensome. We instead drop these duality-based constraints and consider a simpler approach of using the early-stop heuristic to return any feasible point $\tilde\bx^i \in \mX$ found by the solver when the violation $\tilde\bc^i\bhx - \tilde \bc^i\tilde\bx^i$ has exceeded a large number (e.g. $10^{10}$). We find that this early-stop heuristic is almost never called in the experimental section.



==> Tables/LandscapeTable.tex <==
\begin{landscape}	
	\begin{table}[]
		\centering
		\tiny
		\caption{Absolute value results}
		\label{tab:AbsValueResults}
		\begin{tabular}{P{1ex}P{1ex}P{2ex}|P{1ex}P{6ex}P{6ex}|P{1ex}P{6ex}P{6ex}|P{1ex}P{6ex}P{6ex}|P{1ex}P{6ex}P{6ex}|P{1ex}P{6ex}P{6ex}} 
			\multicolumn{3}{c}{}  & 
			\multicolumn{3}{c}{\texttt{K}} & 
			\multicolumn{3}{c}{\texttt{O}} & 
			\multicolumn{3}{c}{\texttt{TD}} & 
			\multicolumn{3}{c}{\texttt{BU}} & 
			\multicolumn{3}{c}{\texttt{Coup}} 
			\\ \hline \Tstrut \Bstrut
			$n$	&	$\nobj$  & $\mathsf{C}$	& $\mathsf{S}$	& $\bar{t}$	& $(\mathsf{M},\mathsf{T})$ 	& $\mathsf{S}$	& $\bar{t}$	& $(\mathsf{M},\mathsf{T})$  	& $\mathsf{S}$	& $\bar{t}$	& $(\mathsf{M},\mathsf{T})$  	& $\mathsf{S}$	& $\bar{t}$	& $(\mathsf{M},\mathsf{T})$  	& $\mathsf{S}$	& $\bar{t}$	& $(\mathsf{M},\mathsf{T})$    \\ \hline \hline \Bstrut\Tstrut
			15 & 3 & 30 & 10 & 1.21   & (0,0)  & 10 & 1.71   & (0,0)  & 10 & 0      & (0,0) & 10 & 0      & (0,0) & 10 & 0      & (0,0) \\
			15 & 4 & 30 & 10 & 8.31   & (0,0)  & 10 & 25.9   & (0,0)  & 10 & 0      & (0,0) & 10 & 0      & (0,0) & 10 & 0      & (0,0) \\
			15 & 5 & 30 & 4  & 1882.3 & (0,6)  & 9  & 2166.9 & (0,1)  & 10 & 0      & (0,0) & 10 & 0      & (0,0) & 10 & 0      & (0,0) \\
			15 & 6 & 30 & 0  & -      & (1,9)  & 0  & -      & (0,10) & 10 & 0      & (0,0) & 10 & 0      & (0,0) & 10 & 0      & (0,0) \\
			15 & 7 & 30 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 0      & (0,0) & 10 & 0      & (0,0) & 10 & 0      & (0,0) \\ \hline \Bstrut\Tstrut
			15 & 3 & 40 & 10 & 2.05   & (0,0)  & 10 & 2.85   & (0,0)  & 10 & 0.01   & (0,0) & 10 & 0.01   & (0,0) & 10 & 0.01   & (0,0) \\
			15 & 4 & 40 & 10 & 23.02  & (0,0)  & 10 & 65.87  & (0,0)  & 10 & 0.01   & (0,0) & 10 & 0.01   & (0,0) & 10 & 0.01   & (0,0) \\
			15 & 5 & 40 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 0.01   & (0,0) & 10 & 0.01   & (0,0) & 10 & 0.01   & (0,0) \\
			15 & 6 & 40 & 0  & -      & (1,9)  & 0  & -      & (0,10) & 10 & 0.02   & (0,0) & 10 & 0.02   & (0,0) & 10 & 0.02   & (0,0) \\
			15 & 7 & 40 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 0.04   & (0,0) & 10 & 0.04   & (0,0) & 10 & 0.04   & (0,0) \\ \hline \Bstrut\Tstrut
			15 & 3 & 50 & 10 & 2.76   & (0,0)  & 10 & 3.71   & (0,0)  & 10 & 0.01   & (0,0) & 10 & 0.01   & (0,0) & 10 & 0.02   & (0,0) \\
			15 & 4 & 50 & 10 & 31.58  & (0,0)  & 10 & 87.62  & (0,0)  & 10 & 0.01   & (0,0) & 10 & 0.02   & (0,0) & 10 & 0.02   & (0,0) \\
			15 & 5 & 50 & 0  & -      & (1,9)  & 0  & -      & (0,10) & 10 & 0.02   & (0,0) & 10 & 0.02   & (0,0) & 10 & 0.02   & (0,0) \\
			15 & 6 & 50 & 0  & -      & (1,9)  & 0  & -      & (0,10) & 10 & 0.03   & (0,0) & 10 & 0.04   & (0,0) & 10 & 0.03   & (0,0) \\
			15 & 7 & 50 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 0.07   & (0,0) & 10 & 0.09   & (0,0) & 10 & 0.05   & (0,0) \\ \hline \Bstrut\Tstrut
			20 & 3 & 30 & 10 & 7.86   & (0,0)  & 10 & 9.84   & (0,0)  & 10 & 0.14   & (0,0) & 10 & 0.14   & (0,0) & 10 & 0.17   & (0,0) \\
			20 & 4 & 30 & 10 & 89.82  & (0,0)  & 10 & 222.09 & (0,0)  & 10 & 0.15   & (0,0) & 10 & 0.14   & (0,0) & 10 & 0.18   & (0,0) \\
			20 & 5 & 30 & 0  & -      & (1,9)  & 0  & -      & (0,10) & 10 & 0.17   & (0,0) & 10 & 0.19   & (0,0) & 10 & 0.21   & (0,0) \\
			20 & 6 & 30 & 0  & -      & (2,8)  & 0  & -      & (0,10) & 10 & 0.24   & (0,0) & 10 & 0.28   & (0,0) & 10 & 0.29   & (0,0) \\
			20 & 7 & 30 & 0  & -      & (1,9)  & 0  & -      & (0,10) & 10 & 0.4    & (0,0) & 10 & 0.49   & (0,0) & 10 & 0.38   & (0,0) \\ \hline \Bstrut\Tstrut
			20 & 3 & 40 & 10 & 32.85  & (0,0)  & 10 & 40.07  & (0,0)  & 10 & 0.63   & (0,0) & 10 & 0.74   & (0,0) & 10 & 0.94   & (0,0) \\
			20 & 4 & 40 & 10 & 553.77 & (0,0)  & 10 & 1046.7 & (0,0)  & 10 & 0.7    & (0,0) & 10 & 0.76   & (0,0) & 10 & 1.06   & (0,0) \\
			20 & 5 & 40 & 0  & -      & (1,9)  & 0  & -      & (0,10) & 10 & 0.8    & (0,0) & 10 & 0.9    & (0,0) & 10 & 1.09   & (0,0) \\
			20 & 6 & 40 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 1.28   & (0,0) & 10 & 1.43   & (0,0) & 10 & 1.56   & (0,0) \\
			20 & 7 & 40 & 0  & -      & (1,9)  & 0  & -      & (0,10) & 10 & 2.62   & (0,0) & 10 & 2.67   & (0,0) & 10 & 2.41   & (0,0) \\ \hline \Bstrut\Tstrut
			20 & 3 & 50 & 10 & 42.55  & (0,0)  & 10 & 55.92  & (0,0)  & 10 & 1.37   & (0,0) & 10 & 1.56   & (0,0) & 10 & 1.98   & (0,0) \\
			20 & 4 & 50 & 10 & 933.77 & (0,0)  & 10 & 1835.4 & (0,0)  & 10 & 1.47   & (0,0) & 10 & 1.69   & (0,0) & 10 & 2.47   & (0,0) \\
			20 & 5 & 50 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 1.84   & (0,0) & 10 & 2.15   & (0,0) & 10 & 2.78   & (0,0) \\
			20 & 6 & 50 & 0  & -      & (2,8)  & 0  & -      & (0,10) & 10 & 3.29   & (0,0) & 10 & 3.5    & (0,0) & 10 & 3.95   & (0,0) \\
			20 & 7 & 50 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 7.08   & (0,0) & 10 & 7.03   & (0,0) & 10 & 6.26   & (0,0) \\ \hline \Bstrut\Tstrut
			25 & 3 & 30 & 10 & 57.61  & (0,0)  & 10 & 69.52  & (0,0)  & 10 & 3.12   & (0,0) & 10 & 3.26   & (0,0) & 10 & 4.21   & (0,0) \\
			25 & 4 & 30 & 10 & 1209.4 & (0,0)  & 9  & 2037.7 & (0,1)  & 10 & 3.35   & (0,0) & 10 & 3.59   & (0,0) & 10 & 4.43   & (0,0) \\
			25 & 5 & 30 & 0  & -      & (1,9)  & 0  & -      & (0,10) & 10 & 3.78   & (0,0) & 10 & 3.98   & (0,0) & 10 & 5.05   & (0,0) \\
			25 & 6 & 30 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 5.69   & (0,0) & 10 & 5.37   & (0,0) & 10 & 7.08   & (0,0) \\
			25 & 7 & 30 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 10.54  & (0,0) & 10 & 8.97   & (0,0) & 10 & 11.03  & (0,0) \\ \hline \Bstrut\Tstrut
			25 & 3 & 40 & 10 & 86.15  & (0,0)  & 10 & 89.88  & (0,0)  & 10 & 24.76  & (0,0) & 10 & 25.68  & (0,0) & 10 & 41.76  & (0,0) \\
			25 & 4 & 40 & 8  & 2974   & (0,2)  & 2  & 3461.5 & (0,8)  & 10 & 26.58  & (0,0) & 10 & 27.51  & (0,0) & 10 & 43.84  & (0,0) \\
			25 & 5 & 40 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 32.49  & (0,0) & 10 & 33.66  & (0,0) & 10 & 51.75  & (0,0) \\
			25 & 6 & 40 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 60.98  & (0,0) & 10 & 51.1   & (0,0) & 10 & 77.37  & (0,0) \\
			25 & 7 & 40 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 148.45 & (0,0) & 10 & 95.4   & (0,0) & 10 & 144.34 & (0,0) \\ \hline \Bstrut\Tstrut
			25 & 3 & 50 & 10 & 87.75  & (0,0)  & 10 & 86.78  & (0,0)  & 10 & 49.21  & (0,0) & 10 & 53.73  & (0,0) & 10 & 99.72  & (0,0) \\
			25 & 4 & 50 & 6  & 2144.1 & (0,4)  & 2  & 2135.3 & (0,8)  & 10 & 54.91  & (0,0) & 10 & 60.58  & (0,0) & 10 & 106.52 & (0,0) \\
			25 & 5 & 50 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 67.79  & (0,0) & 10 & 72.88  & (0,0) & 10 & 128.78 & (0,0) \\
			25 & 6 & 50 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 137.12 & (0,0) & 10 & 111.41 & (0,0) & 10 & 171.18 & (0,0) \\
			25 & 7 & 50 & 0  & -      & (0,10) & 0  & -      & (0,10) & 10 & 427.1  & (0,0) & 10 & 222.51 & (0,0) & 10 & 358.04 & (0,0)
		\end{tabular}
	\label{tab:AbsoluteValueResults}
	\end{table}
	
\end{landscape}


==> Tables/Long_Table.tex <==
\begin{table}[h]
\caption{CP versus CPTR  results.}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{6pt}
{\renewcommand{\arraystretch}{1.01}%
 \begin{tabular}{l r r r r r r r r r r r r}
 \toprule
& \multicolumn{2}{c}{Problem Size} & \multicolumn{2}{c}{CP } & \multicolumn{2}{c}{CP-ES} & \multicolumn{2}{c}{CPTR} & \multicolumn{2}{c}{CPTR-ES} & \multicolumn{2}{c}{CPTR-ES-DR}\\ \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
% & CP &  & CPTR &  & CPTR ES &  & CPTR Stoch ES &  \\
Instance & Vars. & Cons. & It. & Time &  It. & Time & It. & Time & It. & Time & It. & Time\\%[0.3cm]
\hline
50v-10\_t1 & 2013 & 233 & 0 & - & 4964 & - & 1567 & 1919 & 1265 & 206 & 2460 & 370 \\
50v-10\_t2 & 2013 & 233 & 0 & - & 4567 & - & 1002 & 992 & 990 & 121 & 1731 & 240 \\
50v-10\_t3 & 2013 & 233 & 0 & - & 4732 & - & 1456 & 237 & 1351 & 164 & 3046 & 402 \\
assign1-5-8\_t1 & 156 & 161 & 2 & - & 250 & 2061 & 81 & 590 & 81 & 372 & 90 & 266 \\
assign1-5-8\_t2 & 156 & 161 & 4 & - & 71 & 455 & 26 & 38 & 26 & 11 & 26 & 14 \\
assign1-5-8\_t3 & 156 & 161 & 3 & - & 139 & 682 & 50 & 46 & 50 & 47 & 69 & 290 \\
bppc4-08\_t1 & 1456 & 111 & 0 & - & 1 & 108 & 0 & - & 1 & 108 & 1 & 108 \\
bppc4-08\_t2 & 1456 & 111 & 0 & - & 1 & 13 & 0 & - & 1 & 11 & 1 & 11 \\
bppc4-08\_t3 & 1456 & 111 & 0 & - & 1 & 5 & 0 & - & 1 & 5 & 1 & 6 \\
cod105\_t1 & 1024 & 1024 & 5 & - & 6 & - & 10 & - & 17 & 1894 & 27 & 2557 \\
cod105\_t2 & 1024 & 1024 & 0 & 127 & 0 & 121 & 0 & 122 & 0 & 100 & 0 & 117 \\
cod105\_t3 & 1024 & 1024 & 6 & - & 9 & - & 10 & - & 18 & 1474 & 24 & 1916 \\
csched007\_t2 & 1758 & 351 & 3 & - & 256 & - & 20 & - & 147 & - & 144 & 3475 \\
csched008\_t1 & 1536 & 351 & 17 & 1533 & 23 & 260 & 4 & 666 & 5 & 64 & 6 & 91 \\
csched008\_t2 & 1536 & 351 & 17 & 2137 & 115 & 2122 & 10 & 1489 & 40 & 2748 & 41 & 1164 \\
csched008\_t3 & 1536 & 351 & 18 & - & 193 & 2768 & 1 & - & 26 & 130 & 53 & 2711 \\
cvs16r128-89\_t2 & 3472 & 4633 & 0 & - & 489 & - & 6 & - & 200 & 1260 & 270 & 963 \\
cvs16r128-89\_t3 & 3472 & 4633 & 0 & - & 483 & - & 5 & - & 170 & 1368 & 270 & 1680 \\
drayage-100-23\_t1 & 11090 & 4630 & 660 & - & 788 & - & 174 & 245 & 174 & 274 & 195 & 242 \\
drayage-100-23\_t2 & 11090 & 4630 & 935 & - & 755 & 2370 & 124 & 218 & 124 & 247 & 150 & 235 \\
drayage-100-23\_t3 & 11090 & 4630 & 492 & - & 796 & - & 160 & - & 176 & - & 178 & 3520 \\
drayage-25-23\_t1 & 11090 & 4630 & 765 & - & 861 & - & 162 & 277 & 159 & 270 & 173 & 217 \\
drayage-25-23\_t2 & 11090 & 4630 & 912 & 3303 & 875 & 2657 & 129 & 283 & 129 & 321 & 116 & 217 \\
drayage-25-23\_t3 & 11090 & 4630 & 461 & - & 821 & - & 137 & 1069 & 139 & 659 & 172 & 684 \\
eil33-2\_t1 & 4516 & 32 & 89 & 75 & 89 & 71 & 93 & 102 & 104 & 107 & 102 & 102 \\
eil33-2\_t2 & 4516 & 32 & 86 & 101 & 86 & 88 & 87 & 127 & 97 & 142 & 116 & 161 \\
eil33-2\_t3 & 4516 & 32 & 51 & 105 & 52 & 105 & 67 & 405 & 80 & 386 & 93 & 661 \\
enlight\_hard\_t1 & 200 & 100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
enlight\_hard\_t2 & 200 & 100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
enlight\_hard\_t3 & 200 & 100 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\bottomrule
\end{tabular}}}\\%}}\\
\caption{}
\end{table}
